RANK: AI-assisted End-to-End Architecture for Detecting Persistent Attacks in Enterprise Networks

Advanced Persistent Threats (APTs) are sophisticated multi-step attacks, planned and executed by skilled adversaries targeting modern government and enterprise networks. Intrusion Detection Systems (IDSs) and User and Entity Behavior Analytics (UEBA) are commonly employed to aid a security analyst in the detection of APTs. The prolonged nature of APTs, combined with the granular focus of UEBA and IDS, results in overwhelming the analyst with an increasingly impractical number of alerts. Consequent to this abundance of data, and together with the crucial importance of the problem as well as the high cost of the skilled personnel involved, the problem of APT detection becomes a perfect candidate for automation through Artificial Intelligence (AI). In this paper, we provide, up to our knowledge, the first study and implementation of an end-to-end AI-assisted architecture for detecting APTs -- RANK. The goal of the system is not to replace the analyst, rather, it is to automate the complete pipeline from data sources to a final set of incidents for analyst review. The architecture is composed of four consecutive steps: 1) alert templating and merging, 2) alert graph construction, 3) alert graph partitioning into incidents, and 4) incident scoring and ordering. We evaluate our architecture against the 2000 DARPA Intrusion Detection dataset, as well as a read-world private dataset from a medium-scale enterprise. Extensive results are provided showing a three order of magnitude reduction in the amount of data to be reviewed by the analyst, innovative extraction of incidents and security-wise scoring of extracted incidents.

==> intro_old.tex <==
\section{Introduction}

Advanced Persistent Threats (APTs) form a crucial part of the attack campaigns targeting enterprise networks \cite{Ghafir2014}. A combination of stealth actions, sophisticated exploits and long-term operation mark them as one of the most dangerous cybersecurity, and hardest to detect, attacks \cite{mcwhorter2013apt1}. As a planned multi-step attack, APTs do not target a single vulnerability. Instead, an APT typically starts by gaining access to the network, exploiting several vulnerabilities, and remaining silent for extended periods of time \cite{alvarez2017ibm}.  With data exfiltration as the common end-goal of those attacks, the economic damage is particularly severe due to the risk of losing intellectual properties or sensitive data \cite{berghel2017equifax}. Various companies and government agencies have fallen victims to these attacks \cite{rivner2011anatomy, caplan2013cyber}. In light of their severity and impact, detecting APTs has increasingly become the focus of both academia and industry.

A pattern is emerging in the literature where the detection of APTs is composed of numerous small and simple detectors each focused on a single step in the APT chain. Examples of this methodology are \cite{sexton2015attack}, \cite{cao2019preempting}. These small detectors are either based on legacy signature-based intrusion detection systems (IDS), user entity behavior analytics (UEBA) \cite{shashanka2016user}, or a combination of both. However, IDS and UEBA have well-documented problems such as high false-positive ratio, expensive cost of error, difficulty of explainability for anomaly-based detection, lack of training data and continuously improving intelligent adversary \cite{sommer2010outside}. APT-based detection attempts to solve some of those issues, with the main premise being that an alert is malicious if it is part of a larger group of correlated alerts that together represent a proper APT attack plan, significantly reducing the false-positives ratio.


A leading effort to study APT attack plans is the ATT$\&$CK matrix developed by the MITRE corporation \cite{strom2018mitre}. The study observed that attacks tend to follow similar patterns, and provided a taxonomy describing both offensive and defensive operations. The matrix describes the tactics, commonly known as the attack phases, the techniques for carrying out a tactic, and the observed instances of such techniques in known attacks. Our main contribution in this paper is developing an end-to-end architecture for detecting MITRE-aware security incidents. 

In the attempt to detect and reconstruct sophisticated multi-step APTs, individual intrusion alerts are not enough as an indication of compromise \cite{cao2015preemptive}. Instead of individual alerts, more advanced detection approaches try to reconstruct the attack plan \cite{qin2005probabilistic}. In the literature, these approaches can be divided into two broad categories: the first based on Fisher's method for p-value combination \cite{sexton2015attack}; while the second is based on the concept of attack graphs \cite{eshete2016attack}. The first approach of detecting APTs assigns a joint score for multiple detections, and has the advantage of simplicity. However it lacks the sequencing capabilities of attack graphs. In other words, the first approach only considers the coverage of MITRE tactics in the detections, and does not consider whether the order of said detections actually makes sense as an attack plan. Attack graphs are a natural solution here \cite{eshete2016attack}. Besides their visually attractive properties, the topology of a directed graph is a representation of the attack plan progression. In such graphs, each vertex represents an individual alert, which might come from a variety of security solutions, and each edge represents the progression between two alerts \cite{cao2019preempting}.

Despite its attractive properties, an attack graph containing all alerts is usually overwhelmingly large due to the high false-positive rate of the individual alert detectors. This problem can be addressed in two ways. The first approach combines alerts corresponding to the same event together into a Hyper/Generalized alert \cite{julisch2003clustering}, while the second approach works by partitioning the alert graph into smaller sub-graphs. Both approaches result in smaller graphs, reducing the investigation burden on the security analyst. \cite{haas2019alert} is an example of the second approach, where a community-detection approach is proposed with each resulting community corresponding to a single attack step. In \cite{ning2002constructing} alert prerequisites and consequences are defined for each alert to limit the number of edges. Besides the heavy manual work involved, this approach can not handle cases when multiple attacks are carried-out simultaneously. Finally, in \cite{cao2019preempting} a separate graph is defined for each single asset. This approach results in manageable graphs, but it ignores lateral movement, a common tactic in APT attacks. However, community detection algorithms focus only on the graph's topological properties, and fail to incorporate security context to determine whether a community represents an actual attack plan or not. Part of the proposed architecture is a novel graph partitioning capable of extracting more meaningful incidents from alert graphs.

It is worth emphasizing again the difference between the two main approaches in reducing the size of the graph, the first approach tries to combine together alerts corresponding to the same step in APT into a single alert, equivalent to a node in the graph. The second approach aims at collecting all steps for a single coherent APT into a separate subgraph representing the incident. Identifying the difference between the two approaches and having them work together in the same architecture is an important contribution of this work.

In this paper, we propose RANK, an end-to-end architecture for detecting persistent attacks. The architecture is composed of several steps, starting with alert templating and merging, followed by alert graph construction and partitioning into concise incidents, before finally building a factor graph (FG) for each incident to calculate its final score. Moreover, we also discuss how the MITRE tactics can be incorporated into the alert graph construction and partitioning, as well as the scoring step. The proposed architecture is also able to integrate analyst feedback as part of incident investigation and hunting. This is enabled by the evidence-based queries provided by the scoring factor graph for each incident. In particular, our contributions in this paper are:
\begin{itemize}
    \item We propose the first, up to our knowledge, architecture for end-to-end detection of persistent attacks from network and endpoint data.
    \item We discuss various practical aspects of the involved algorithms, such as meaningful clustering of security alerts, calculating correlation between IP addresses, and building all the algorithms with minimal manual tweaking effort due to the lack of labelled datasets.
    \item We discuss a novel approach for the graph partitioning into separate incidents and how it fits into the architecture, part of which is also published in \cite{Soliman2020}.
    \item We discuss a horizontally-scalable implementation of the proposed architecture which is currently deployed in production systems, and the various components needed to build it.
\end{itemize}

==> software.tex <==
\section{Scalable Software Architecture}

% I went through a few iterations of this, unsure of the focus. This
% verison highlights the "scalable" part of the section title,
% mentioning tech details when they pertain to scalability:
% streaming/batch and partitioning.

The process of converting alerts into discrete incidents, each
composed of multiple generalized alerts, is implemented in three main
steps:

\begin{itemize}
   \item Learning alert templates from batches of alerts
   \item Processing alerts as they are created and merging them into generalized alerts
   \item Constructing alert graphs from batches of generalized alerts, partitioning them into incident graphs, and scoring the incidents
\end{itemize}

The first and third steps, learning alert templates and extracting the
incidents, are both implemented as independent batch jobs using
Spark\footnote{\url{https://spark.apache.org/}} to distribute work
over a cluster of workers. The second stage, generalizing alerts,
occurs in long-running Java processes that use
Kafka\footnote{\url{https://kafka.apache.org/}} topics to communicate
and partition alerts and generalized alerts.

A primary concern of the implementation is ensuring each step is
scalable. The work should be distributable across multiple threads and
multiple machines so that the overall solution can scale up to handle
an increasing volume of alerts from an increasing number of
sources. Similarly the inputs to and outputs from each step should be
distributed and partitioned to avoid bottlenecks.

\subsection{Learning Alert Templates}

The first batch job learns the templates from a set of ungeneralized
alerts. This is the ``Template Extraction'' step shown in
Fig. \ref{fig:architecture}. This step reads a potentially large
number of alerts from a data store, which can be costly. Fortunately,
not every alert needs to be read and the required computation,
described in Section \ref{sec:template}, is relatively
inexpensive. Additionally, given the same set of alert sources, there
is the opportunity to share learned alert templates across systems
monitoring different networks. We are still experimenting with the
input interval and run frequency of this step.

The output is the alert templates, which are made available to all
processes performing the alert generalization. This data is relatively
small and rarely changes, so it is not difficult to distribute.

\subsection{Generalizing Alerts}

Every alert in the monitored system must be generalized according to
the learned templates so that it has the opportunity to contribute to
one or more incidents. Alerts enter the system in a streaming, online
manner, before being written to a data store. Rather than reading all
alerts out of the data store again to generalize them, which would be
costly, this step is implemented as a streaming task, labelled ``Alert
Merging'' in Fig. \ref{fig:architecture}.

% Could further motivate why this part is streaming by reiterating the
% order of magnitude reduction from alerts to generalized alerts.

As each alert is generated, the subset of information about the alert
needed for incidents is published to a topic partitioned by the
alert's source, which is the same partitioning used by the alert
templates; alerts from different sources cannot be merged together
during generalization. A set of long-running Java processes consume
that topic, using the learned alert templates to determine the
generalized alert that each incoming alert belongs to.

The alerts are merged into generalized alerts stored in a key-value
store provided by Kafka
Streams\footnote{\url{https://kafka.apache.org/documentation/streams/}}. Beyond
providing a fast local key-value store for each process, the store
also publishes a change log to another Kafka topic. This change log
has compaction enabled and a retention time, allowing it to
effeciently store the latest value for each merged generalized alert
within a recent time interval. The change log allows restarting the
process on another machine and also serves as the input to the
incident extraction in the subsequent step.

\subsection{Extracting Incidents}

Incident extraction is the most complex of the three steps. It is a
multi-stage Spark batch job which reads the compacted change log of
generalized alerts. The retention time of the topic determines the
time interval of alerts being considered, although additional
filtering can be done if smaller intervals are desired.

Alert graphs are constructed, partitioned into incident graphs, and
scored as described in Sections
\ref{sec:corrgraph}--\ref{sec:scoring}. All of the graphs are
represented and processed using Spark
GraphX\footnote{\url{https://spark.apache.org/graphx/}} to maintain
scalability. Currently, the graph partitioning is performed using the
more scalable community detection approach rather than the convex
optimization approach.

% remove this line?
The resulting scored incidents are output for analyst review.

% \subsection{Future Direction}

% unsure if this part should be in the paper at all or if it should be
% moved to Future Work

% Further development will focus on updating incidents, both to
% incorporate analyst feedback and to potentially add additional alerts
% as they occur. Both of these improvements will likely move some
% aspects of the incident extraction and scoring from a batch to a
% streaming context where the resulting updated incidents will be more
% readily available to analysts.

